Gravity at the Tip of the Throat

We study the gravitational signatures that arise from compactifying Type IIB supergravity on a compact space containing a Klebanov-Strassler warped throat. After reviewing the dimensional reduction of the 10d graviton and explicitly obtaining the equations of motion for the 4d tensor $h_{\mu\nu}$, vector $h_{\mu n}$ and scalar $h_{mn}$ modes, we find the masses and wavefunctions of the Kaluza-Klein tower of spin-2 states. We explore how the masses and wavefunctions depend on the balance between the strength of the warping and the size of the bulk, and how these relate to the range and strength of the interactions which correct the Newtonian gravitational potential. By computing the modified Newtonian potential for sources on a brane somewhere along the throat, and applying consistency constraints on the Klebanov-Strassler parameters, we obtain predictions for the phenomenological parameter space. In the case of a fully warped throat, and depending on where the brane is along the throat, these predictions are narrow in range and consistent with current observational and experimental constraints. We also begin an exploration of gravitational wave signatures of KK gravitons in warped throats, finding that strong warping can bring the corresponding frequencies down to the windows of current and proposed experiments.

==> Sections/compactification.tex <==
\subsection{Background solution - the warped deformed conifold}
\label{sec:4dEFT_compactification}

\def\rs{r_{\ll}}
\def\rl{r_{\gg}}

In order to obtain the 4d EFT, we consider a Type IIB flux compactification with an internal space composed of a compact CY$_3$, which constitutes the bulk of the compact space, together with a warped throat, which can be described by the Klebanov-Strassler solution \cite{KS2000supergravity}, corresponding to a warped deformed conifold\footnote{The Klebanov-Strassel solution is a special case of a broader class of solutions for the deformation of the conifold metric with fluxes that preserve the $SU(2)\times SU(2)\times\Z_2$ symmetry of the geometry \cite{PTconifold}.}, smoothly glued to the bulk. Considering surfaces in $\C^4$ given by $\sum_{i=1}^4 w_i^2 = \epsilon^2$, with $\epsilon$ a non-zero complex parameter (if $\epsilon=0$ the conifold is singular), gives a deformed conifold with metric \cite{candelas1990conifolds,Minasian:1999tt,Aganagic:1999fe,KS2000supergravity} 
%
\begin{align}
    ds_{con}^2 = \frac{\epsilon^{4/3}}{2}\mathcal{K}(\tau) 
    \Bigg( \frac{1}{3\mathcal{K}^3(\tau)} \left(d\tau^2 + (g^5)^2 \right) 
    &+ \sinh^2(\tau/2) \left( (g^1)^2 + (g^2)^2 \right) \nonumber \\
    &+ \cosh^2(\tau/2) \left( (g^3)^2 + (g^4)^2 \right)
    \Bigg) \,,
    \label{eq:conifold:deformed_conifold_metric}
\end{align}
where $\mathcal{K}(\tau) = \frac{(\sinh(2\tau) - 2\tau)^{1/3}}{2^{1/3}\sinh(\tau)}$ and $g^i$ are a basis of one-forms \cite{candelas1990conifolds}. In this basis, the metric written only depends on $\tau$ which is related to the radial direction along the cone. 
%
For large $\tau$ the metric approaches the singular conifold metric
\begin{align}
    ds_{con}^2 
    &= d\rl^2 + \rl^2\left(\frac{1}{9}(g^5)^2 +\frac{1}{6}\sum_{i=1}^{4}(g^i)^2 \right),
    \quad \text{ as } \tau\to\infty \,,
    \label{eq:metric_conifold_largetau}
\end{align}
%
where the coordinate $\rl$ is defined as $\rl^2 = \frac{3}{2^{5/3}}\epsilon^{4/3}e^{2\tau/3}$, while for small $\tau$
\begin{align}
    ds_{con}^2 
    &= d\rs^2 + \frac{\rs^2}{8}d\mathrm{\Omega}_2^2 + R_\epsilon^2 d\mathrm{\Omega}_3^2,
    \quad \text{ as } \tau\to 0 \,,
    \label{eq:metric_conifold_smalltau}
\end{align}
%
where $\rs^2 = \frac{\epsilon^{4/3}}{4}\left(\frac{2}{3}\right)^{1/3}{\tau}^2$, $d\mathrm{\Omega}_2^2=((g^1)^2+(g^2)^2)$ is the metric of an $S^2$ and $d\mathrm{\Omega}_3^2=((g^3)^2+(g^4)^2+\frac{1}{2}(g^5)^2)$ is the metric of an $S^3$. We see that $\rs\rightarrow 0$ as $\tau\rightarrow 0$, and we are left with the metric for an $S^3$ whose size $R_\epsilon$ is controlled by the deformation parameter $\epsilon$,
%
\begin{align}
    R_\epsilon^2 = \frac{\epsilon^{4/3}}{2}  \left(\frac{2}{3}\right)^{1/3} \,.
\end{align}

The Klebanov-Strassler solution is obtained in \cite{KS2000supergravity}, using the deformed conifold as an ansatz for the internal space of a warped solution of Type IIB supergravity. The 10d metric can be written as
\begin{align}
    ds_{10}^2 &= e^{2A} g_{\mu\nu}dx^{\mu}dx^{\nu} + e^{-2A} g_{mn}dy^mdy^n \,.
    \label{eq:metric}
\end{align}

Notice that this results in a non-compact solution, which is not suitable for phenomenological applications. Therefore, in practice only a finite portion of the Klebanov-Strassler solution is used and glued to a compact CY$_3$ (or more generally, a compact 6d \textit{bulk}). Due to the symmetries of the conifold, the warp factor can only depend on $\tau$ and is given by \cite{KS2000supergravity}
%
\begin{align}
    e^{-4A} &=
    2^{2/3}\frac{(\alpha' g_sM)^2}{\epsilon^{8/3}} I(\tau) \,,
    \quad\quad I(\tau)\equiv \int_{\tau}^{\infty} dx ~ \frac{x\coth(x) - 1}{\sinh^2{x}}(\sinh(2x)-2x)^{1/3} \,. 
    \label{eq:deformedConifold_warpfactor}
\end{align}

For the conifold in the small $\tau$ limit the metric takes the form
\begin{align}
    ds_{10}^2 
    = e^{2A} g_{\mu\nu}dx^{\mu}dx^{\nu} + e^{-2A} \left(d\rs^2 + \frac{\rs^2}{8}d\mathrm{\Omega}_2^2 + R_\epsilon^2 d\mathrm{\Omega}_3^2 \right).
\end{align}

\noindent The physical size of the $S^3$ is $R^2_{S^3}=e^{-2A}R_\epsilon^2$, which does not depend on the deformation parameter $\epsilon$
%
\begin{align}
    R_{S^3}^2 &= e^{-2A} R_\epsilon^2
    = \left(\frac{2^{2/3}}{3^{1/3}} I^{1/2}(\tau)\right)(g_sM)\alpha' 
	\overset{\tau = 0}{\approx} (g_s M)\alpha' \,,
\end{align}
%
from which follows the condition $g_sM\gg 1$ for a well under control supergravity (i.e. such that the $\alpha'$-expansion with which the Type IIB low-energy supergravity used in \cite{KS2000supergravity} is derived is under control).

Far away from the tip, the warp factor becomes \cite{KT}
\begin{align}
	e^{-4A} \approx \frac{L^4}{\rl^4}\left[1 + \frac{3 g_sM}{8\pi K} + \frac{3g_s M}{2\pi K}\log\Big(\frac{\rl}{r_{UV}}\Big) \right] \,,
	\label{E:mouthwarp}
\end{align}
where we define 
\begin{align}
	L^4 = \frac{27\pi}{4}\frac{g_sMK}{(2\pi)^4}~l_s^4 .
\end{align}
with $K$ being the flux number through the non-compact cycle\footnote{More precisely, the cycle which is non-compact in the non-compact Klebanov-Strassler solution, but becomes compact when only a finite portion is glued to the compact bulk.} and $r_{UV}$ the value of $\rl$ where we cut the throat and glue it to the bulk
%\footnote{We call it $r_{UV}$ because the warping which creates the warped throat also creates a hierarchy between the tip of the throat (IR) and the bulk (UV) from the 4d point-of-view. Once $r_{UV}$ is reached, the warp factor is no longer relevant and the energy scales in the 4d theory at those points in the compact space are no longer suppressed with respect to the natural (UV) scale of the theory.},
\begin{equation}
	r_{UV} \equiv \frac{3^{1/2}}{2^{5/6}}\epsilon^{2/3}e^{\tau_{UV}/3} \,.
	\label{eq:rUV}
\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DO WE WANT THE ASYMPTOTIC EXPRESSIONS IN DETAIL? 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse.
We present here the $\tau\to 0,\infty$ limits of the functions $\mathcal{K}(\tau)$ and $I(\tau)$ will be useful in what follows,
\begin{align}
    &\mathcal{K}(\tau\to 0) \to \left(\frac{2}{3}\right)^{1/3} + \Op(\tau^2) \,, 
    &&I(\tau\to 0) \to a_0 + \Op(\tau^2) \,,
    \label{eq:conifoldFunctionsSmallTau} \\ 
    &\mathcal{K}(\tau\to\infty) \to 2^{1/3}e^{-\tau/3} \,, 
    &&I(\tau\to\infty) \to \frac{3}{2^{1/3}}\left(\tau + \frac{3}{4}\right)e^{-4\tau/3}  \,.
    \label{eq:conifoldFunctionsLargeTau}
\end{align}
as well as the determinant
%
\begin{align}
    \det g_{con} = \frac{\epsilon^8}{3^2\cdot 2^{10}}\sinh^4(\tau) \,.
\end{align}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The background warp factor, $e^{-4A}$, that solves the 10d Einstein equations in the presence of fluxes, is only fixed up to a constant shift in $y^m$, motivating the following form \cite{frey2009universal}
\begin{equation}
    e^{-4A(y)} = e^{-4A_0(y)} + c(x).
\end{equation}
On the other hand, $g_{mn}\rightarrow\lambda g_{mn}$ together with $e^{2A}\rightarrow \lambda e^{2A}$ is a gauge redundancy of the 6d part of the metric \cite{Giddings:2005ff,Aparicio:2015psl}, and we can choose $\lambda=c(x)^{1/2}$ to rewrite (\ref{eq:metric}) as
%
\begin{equation}
    ds^2 
    = \left[1 + \frac{e^{-4A_0(y)}}{c(x)}\right]^{-1/2} e^{2\mathrm{\Omega}(x)} g_{\mu\nu}dx^{\mu}dx^{\nu}  + \left[1 + \frac{e^{-4A_0(y)}}{c(x)}\right]^{1/2}  c(x)^{1/2} g_{mn}dy^mdy^n \,,
    \label{eq:10dmetric_ourconventions}
\end{equation}
%
and define the warp factor as 
\be\label{WF}
H=1+\frac{e^{-4A_0(y)}}{c(x)} \,.
\ee
In the limit $c(x)\rightarrow\infty$, $H\to 1$ and we naturally recover the unwarped case. Approaching that limit we identify $c(x)=\mathcal{V}^{2/3}$, where $\mathcal{V}\,l_s^6$ is the unwarped volume of the compact space, as we would expect for a volume modulus once coordinates are chosen such that $V_{6} = \int d^6y\sqrt{g_6} = l_s^6$. The factor $e^{2\mathrm{\Omega}(x)}$ anticipates the Weyl-rescaling necessary to go to the Einstein frame in 4d. 

Importantly, the question of whether a region is warped, through $H(\tau)$, depends not only on the solution $e^{-4A_0(\tau)}$, but also on the size of the bulk to which the throat is glued. The warping will dominate when $e^{-4A_0(\tau)}\gg c$ and be negligible when $e^{-4A_0(\tau)}\ll c$, so that effectively the throat ends at $e^{-4A_0(\tau)}\sim c$. This interplay between $e^{-4A_0(\tau)}$ and $c$ gives an interesting intermediate regime of weak warping which was explored in \cite{Bento:2021nbb}. For concreteness, we can define the gluing point $\tau_c$ such that $e^{-4A_0(\tau_c)} = c$, keeping in mind that the gluing must involve a smooth transition between the warped throat and the bulk around $\tau_c$. 
%\footnote{Note that in the throat, when $e^{-4A_0(\tau)}\gg c$, we exactly recover the 6d part of (\ref{eq:metric}), 
%%since $\left[1 + \frac{e^{-4A_0(y)}}{c(x)}\right]^{1/2}  c(x)^{1/2} g_{mn}dy^mdy^n \approx e^{-4A_0(y)}g_{mn}dy^mdy^n$, 
%while for the bulk, when $e^{-4A_0(\tau)}\ll c$, 
%%$\left[1 + \frac{e^{-4A_0(y)}}{c(x)}\right]^{1/2}  c(x)^{1/2} g_{mn}dy^mdy^n 
%we recover the usual form of an unwarped compactification $ds_6^2\approx c(x)^{1/2} g_{mn}dy^mdy^n$. 
%The relevant difference is in the 4d part of the metric, where in the bulk 
%%we have $\left[1 + \frac{e^{-4A_0(y)}}{c(x)}\right]^{-1/2} e^{2\Omega(x)} g_{\mu\nu}dx^{\mu}dx^{\nu} 
%(\ref{eq:10dmetric_ourconventions}) gives $ds_4^2\approx g_{\mu\nu}dx^{\mu}dx^{\nu}$ and (\ref{eq:metric}) gives $ds_4^2\approx c^{1/2}(x) g_{\mu\nu}dx^{\mu}dx^{\nu}$. While the former gives the well-known relation identification $\V = c^{3/2}$, the latter would give $\V = c$.}
%
Therefore $\tau_c$ can be defined implicitly in terms of the conifold parameters
%and the warp factor for the deformed conifold (\ref{eq:deformedConifold_warpfactor}),
\begin{equation}
	\frac{e^{-4A_0(\tau_c)}}{c} = 1 \implies 2^{2/3}\frac{(\alpha' g_s M)^2}{c~\epsilon^{8/3}} = \frac{1}{I(\tau_c)}\,, 
	\label{eq:tauc_parameters}
\end{equation}
which allows us to rewrite the warp factor as
\begin{equation}
	H_{\tau_c}(\tau) = 1 + \frac{I(\tau)}{I(\tau_c)} \,.
	\label{eq:warp_factor_tauc}
\end{equation}

\begin{figure}[t]
     \centering
	\begin{subfigure}[b]{0.48\textwidth}
        	\centering
         	\includegraphics[width=\textwidth]{Plots/warp_factor_tauc.pdf}
     	\end{subfigure}
     \hfill
	\begin{subfigure}[b]{0.48\textwidth}
        	\centering
         	\includegraphics[width=\textwidth]{Plots/warp_factor_large_tauc.pdf}
     	\end{subfigure}
    \caption{Warp factor $H(\tau)$ (in log scale) for different choices of $\tau_c$. We can see how the choice of $\tau_c$ is directly related to the strength of the warping and the size of the warped throat (defined has the region with non-trivial warping).}
    \label{fig:warp_factor}
\end{figure}

\noindent This highlights the fact that the warp factor depends on one parameter only, $\tau_c$. Even though it is implicitly determined by a specific combination of the more familiar parameters through (\ref{eq:tauc_parameters}), it is a convenient parametrisation since a choice of $\tau_c$ has a clear physical interpretation. In Fig.\ref{fig:warp_factor} we show how the warp-factor $H(\tau)$ behaves for different choices of $\tau_c$.  



Dimensionally reducing the 10d Einstein-Hilbert term in (\ref{eq:TypeIIB_action_EinsteinFrame}) down to 4d using the metric (\ref{eq:10dmetric_ourconventions}), we obtain
\begin{equation}
    S  = \frac{V_w^0}{2\kappa^2}\int d^{4}x \sqrt{-g_4}  R_4 + ... \,,
    \label{eq:dimRed_kineticTerms}
\end{equation}
where the Weyl factor $e^{2\mathrm{\Omega}(x)}$ is defined as 
%
\begin{equation}
    	e^{2\mathrm{\Omega}(x)} = \frac{V_w^0}{c(x)^{3/2}\int d^6y \sqrt{g_6} ~H} = \frac{V_w^0}{V_w} \,,
    	\quad V_w = ~c(x)^{3/2}\int d^6y \sqrt{g_6} ~H\,.
	\label{eq:Vw_definition}
\end{equation}
%
The choice of constant $V_w^0$, which ensures that the Weyl factor is dimensionless, is arbitrary\footnote{Note that all the mass-scales in units of $M_{p}$ will be independent of the normalisation of $e^{2\mathrm{\Omega}(x)}$.}. The most convenient choice is $V_w^0 \equiv \langle V_w \rangle$, such that $\langle e^{2\mathrm{\Omega}(x)}\rangle =1$, i.e. the two frames are the same at the vev and we can relate the string scale with the 4d Planck scale using frame independent volumes.  With this choice, the definition of $M_P$ is
\begin{equation}
    \frac{M_P^2}{2} = \frac{1}{2\kappa_4^2} = \frac{V_w^0}{2\kappa^2}
	\implies
	\frac{m_s}{M_P} = \frac{g_s}{\sqrt{4\pi\V_w^0}} \,.
	\label{eq:msMp}
\end{equation}
Note that the relation between the string scale\footnote{In our conventions, $(2\pi)^2\alpha' = l_s^2$ and $m_s=l_s^{-1}$, which differs from $M_s=1/\sqrt{\alpha'} = 2\pi m_s$.} and the 4d Planck scale is only determined once the volume modulus is fixed (analogously to what happens with the dilaton in 10d, where the physical gravitational coupling can only be related to the string frame coupling once the dilaton is fixed). In what follows we assume that all moduli are stabilised, including in particular the volume modulus, and work at the resulting vacuum. Therefore, we use the metric 
\begin{equation}
    ds^2 
    = H^{-1/2} g_{\mu\nu}dx^{\mu}dx^{\nu}  + H^{1/2}  c^{1/2} g_{mn}dy^mdy^n \,,
    \label{eq:10dmetric}
\end{equation}
by setting $e^{2\mathrm{\Omega}(x)}$ to its value at the vacuum and letting $c=\langle c(x)\rangle$ and $V_w = V_w^0$ from now on. 
%If the bulk region of the compact space dominates0 the volume integral in the definition of $V_w$ (\ref{eq:Vw_definition}) so that $V_w\approx \V l_s^6$, the string and Planck scales are related as 
%\be\label{eq:msMp}
%	\frac{m_s}{M_P} = \frac{g_s}{\sqrt{4\pi\V}}\,.
%\ee

%In the limit of small warping (or for no warping at all), where $c(x)\gg e^{-4A_0(y)}$ and $H\approx 1$ for most of the internal space, we have $V_w^0 = \V_w^0 l_s^6 \approx \langle\mathcal{V}\rangle l_s^6$, the physical volume of the compact space.

For the simple case we are considering, with one bulk and one throat, $V_w$ is the sum of the bulk volume $V_\mathcal{B}$ and the throat volume $V_{th}$, 
\be\label{eq:Vw_total}
	V_w = V_{\mathcal{B}} + V_{th} \,,
\ee
where
\begin{align}
	V_{\mathcal{B}} &\approx c^{3/2}\int_{bulk} d^6 y \sqrt{g_6} = c^{3/2} l_s^6 \,,
	\label{eq:V_Bulk}
\end{align}

\noindent whereas for $V_{th}$ we find
\begin{align}
	V_{th} &\approx c^{1/2}\int_{throat} d^6y \sqrt{g_6} e^{-4A_0(y)} \nonumber \\
	&= 2^{5/3}\frac{\pi^3}{3}\frac{(\alpha'g_sM)^2}{\epsilon^{8/3}}\epsilon^4c^{1/2} \int_0^{\tau_c} d\tau \sinh^2(\tau) I(\tau) \nonumber \\
	&\approx\frac{9\pi^3}{16\cdot 2^{1/3}}\frac{(\alpha'g_sM)^2}{\epsilon^{8/3}}\epsilon^4c^{1/2}  \left\{1 + e^{2\tau_c/3}\Big(\frac{2}{3}\tau_c -1\Big) \right\} \,,
\end{align}
where we used the large $\tau$ behaviour of the integrand to perform the integral. Expressing this in terms of $r_{UV}$ (\ref{eq:rUV}), using the flux quantisation condition that defines the flux number $K$ and the fact that $\frac{2\pi K}{g_sM}\gg 1$, we find
\be\label{eq:V_throat}
	V_{th} \approx 2\pi^4 g_s M K (\alpha')^2 c^{1/2} r_{UV}^2 = \frac{g_s MK}{8}\Big(\frac{R_{throat}}{l_s}\Big)^2 ~ l_s^6 \,,
\ee
where we defined the physical size of the throat, $R_{throat} = c^{1/4} r_{UV}$.
This can be compared with the volume of the unwarped deformed conifold of physical size $R_{con}$, 
\be\label{eq:V_uwarped_conifold}
	V_{con} = \frac{(2\pi)^3}{81}\left(\frac{R_{con}}{l_s}\right)^6 ~ l_s^6\,.
\ee

\iffalse
Putting these together, we find
\be\label{eq:Vw_total_explicit}
	\V_w \approx c^{3/2}\left(1 + \frac{g_s MK}{8c^{3/2}}\Big(\frac{r_{UV}}{l_s}\Big)^2 \right) \,. 
\ee
\fi

Our goal is to find the towers of KK modes that follow from the 10d metric after compactifying the Type IIB action on the background geometry (\ref{eq:10dmetric}) and identify their effects on 4d gravitational interactions. In the next subsection we decompose the wave equation (\ref{eq:10dWaveEq}) using the background (\ref{eq:10dmetric}) and find the equations for infinite towers of 4d tensor, vector and scalar modes. 
